Preference-Based Abstract Argumentation for Case-Based Reasoning (with Appendix)

In the pursuit of enhancing the efficacy and flexibility of interpretable, data-driven classification models, this work introduces a novel incorporation of user-defined preferences with Abstract Argumentation and Case-Based Reasoning (CBR). Specifically, we introduce Preference-Based Abstract Argumentation for Case-Based Reasoning (which we call AA-CBR-P), allowing users to define multiple approaches to compare cases with an ordering that specifies their preference over these comparison approaches. We prove that the model inherently follows these preferences when making predictions and show that previous abstract argumentation for case-based reasoning approaches are insufficient at expressing preferences over constituents of an argument. We then demonstrate how this can be applied to a real-world medical dataset sourced from a clinical trial evaluating differing assessment methods of patients with a primary brain tumour. We show empirically that our approach outperforms other interpretable machine learning models on this dataset.

==> aa-cbr-p-def.tex <==
Here we present again the definitions of \aacbrp~so that they can be referred to in the rest of the supplementary material.

\begin{manualdefinition}{4}[Preference Ordering]
% \improvement{Explain why Preorder not a partial order (maybe a footnote) \gppnew{GPP: yes!}}
    Let \mbox{$\pseq$ = $\langle \succcurlyeq_{1}, \ldots, \succcurlyeq_n \rangle$} be a sequence of preorders, each defined over $X$. Each preorder, $\succcurlyeq_{i}$, is a reflexive and transitive relation, with a corresponding strict preorder, $\succ_{i}$ (which is irreflexive and transitive), and an equivalence relation, $=_{i}$ (which is reflexive, symmetric, and transitive). For cases $\casealpha, \casebeta  \in D \cup \{\casedefault \}$, we define:
    \begin{itemize}

        \item $\xalpha \succ_{i} \xbeta $ iff $\xalpha \succcurlyeq_{i} \xbeta$ and $\xbeta \not \succcurlyeq_{i} \xalpha$  

        \item $\xalpha =_{i} \xbeta$ iff $\xalpha \succcurlyeq_{i} \xbeta$ and $\xbeta \succcurlyeq_{i} \xalpha$

    \end{itemize}

\end{manualdefinition}



\begin{manualnotation}{1}[Shorthand Notations]
We use $\xalpha \bigsucccurlyeq{j}{k} \xbeta$, where $j \leq k$, to mean $\xalpha$ is equivalent or larger than $\xbeta$ on all preorders between orders $\succcurlyeq_{j}$ and $\succcurlyeq_{k}$ (inclusive). 
This is defined as:
\begin{align*}
\xalpha \bigsucccurlyeq{j}{k} \xbeta \text{ iff } \forall i \in [j, k], \xalpha \succcurlyeq_{i} \xbeta. 
\end{align*}

\noindent
Shorthands for $\bigeq{j}{k}$ and $\bigsucc{j}{k}$ are defined analogously.

    % \item Let $\xalpha \bigeq{j}{k} \xbeta$ iff $\forall i \in [j, k] $, $\xalpha =_{i} \xbeta$;
    % \item Let $\xalpha \bigsucc{j}{k} \xbeta$ iff $\forall i \in [j, k]$, $\xalpha \succ_{i} \xbeta$;
    % \item Let $\xalpha \bigsucccurlyeq{j}{k} \xbeta$ iff $\forall i \in [j, k]$, $\xalpha \succcurlyeq_{i} \xbeta$;
\end{manualnotation}



\begin{manualdefinition}{5}[Potential Attacks] Let $\alpha = \casealpha$ and $\beta = \casebeta$. For $\alpha, \beta \in D \cup \{ \casedefault \}$, we define a \emph{potential attack} on order $\succcurlyeq_{i}$ as: $\alpha \potentialattacks{i} \beta$ iff

    \begin{enumerate}[i]
        \item $y_{\alpha} \neq y_{\beta}$, and
        \item $\xalpha \succ_i \xbeta$, and
        \item $\xalpha \bigeq{1}{i-1} \xbeta$.
    \end{enumerate}
\label{def:potential-attacks}
\end{manualdefinition}



\begin{manualdefinition}{6}[Casebase Attacks] 
Let $\alpha = \casealpha$ and $\beta = \casebeta$.
For $\alpha, \beta \in D \cup \{ \casedefault \}$, we define an attack on order $\succcurlyeq_{i}$: $\alpha \attacks[i] \beta$ iff
    \label{def:specificity-attacks}

    \begin{enumerate}[i]
        \item $\alpha \potentialattacks{i} \beta$ and
        \item $\nexists \gamma = \casegamma \in D \cup \{ \casedefault \}$ with $\xalpha \bigsucccurlyeq{1}{n} \xgamma$ and
              \begin{enumerate}
              
                  \item either $\gamma \potentialattacks{i} \beta$ and $\exists l \geq i,$ $\xalpha \succ_{l} \xgamma$, 
                  
                  \item or $\gamma \not \potentialattacks{i} \beta$ and $\exists l > i,$ $\gamma \potentialattacks{l} \beta$. 
                  
              \end{enumerate}
    \end{enumerate}
\end{manualdefinition}



\begin{manualdefinition}{7}[Coherent and Incoherent Casebases]

A casebase $D$ is \emph{coherent} iff there are no two cases $\casealpha, \casebeta \in D$ such that $\xalpha \bigeq{1}{n} \xbeta$ and $y_{\alpha} \not = y_{\beta}$, and it is \emph{incoherent} otherwise.
\end{manualdefinition}




\begin{manualdefinition}{8}[Incoherent Attacks] 
\label{incoherent-attacks}
For $\casealpha, \casebeta \in D \cup \{\casedefault\}$, we define an incoherent attack: $\casealpha \incoherentattacks \casebeta$ iff $\xalpha \bigeq{1}{n} \xbeta$ and $y_{\alpha} \neq y_{\beta}$.

\end{manualdefinition}


\begin{manualdefinition}{9}[New Case Attacks] 
\label{new-case-attacks}
For $\casealpha \in D \cup \{\casedefault\}$ and new case $N = \casenew$, we define a new case attack: $N \newattacks \casealpha$ iff $N \nsim \casealpha.$

\end{manualdefinition}



\begin{manualdefinition}{10}[] The argumentation framework \afp{N} mined from dataset $D$ and a new case $N$, with a sequence of preorders $\pseq$ of length $n$ is $(Args, \attacks)$ where
\label{def:aa-cbr-p}

\begin{itemize}
    \item[] $Args = D \cup \{\casedefault\} \cup \{N\}$ and
    \item[] \mbox{$\attacks = (\bigcup_{i=1}^{n} \attacks[i]) \cup \incoherentattacks \cup \newattacks$}.
\end{itemize}

\end{manualdefinition}


\begin{manualdefinition}{11}[Regular]
\label{def:regular-aa-cbr-p}
    The AF mined from $D$ and $N$, with default argument $\casedefault$ is \emph{regular} when:

    \begin{enumerate}
        \item The irrelevance relation $\nsim$ is defined as $\xalpha \nsim \xbeta$ iff $\exists i, \xalpha \not \succcurlyeq_{i} \xbeta$.
        \item $\x{\delta}$ is the least element on all orders in $\pseq$.
    \end{enumerate}

\end{manualdefinition}




==> explanation.tex <==
% \todoin{
% \begin{itemize}
    % \item Dispute Trees
    % \begin{itemize}
    %     \item Define a dispute tree
    %     \item Give an example of a dispute tree
    %     \item Note: for a coherent casebase, a dispute tree must exist. Use coherent casebase = acyclic graph. (W-root if  AA-CBR-$P_{\succcurlyeq}(D, x_{n}) = \delta$ and L-root otherwise) -> Not sure if this is true anymore 
    %     \item  
    % \end{itemize}
% \end{itemize}
% }


The explanations of an outcome predicted by \mbox{AA-CBR-$P_{\succcurlyeq}$} follow a dialectical conversation between two players, $W$ (winner) and $L$ (loser). $W$ argues in favour of the outcome assigned to $N$, whilst $L$ refutes this. The debate starts with one of the players proposing that $\casedefault$ should hold for $N$. If $y_{N} = \delta$, then $W$ is the one who starts the debate; otherwise, $L$ does. The next player can then refute this using an attacker of the default case in the AF. The players then take turns to refute the other's arguments until $L$ no longer refutes $W$'s arguments. This dialectical exchange can be represented as an \textit{arbitrated dispute tree}~\cite{arbitrated-argumentative-dispute}.
\unsure{Explanations by arbitrated argumentative dispute discusses the suitability of dispute trees in their related works section - might need to do something similar or refer to their discussion?}

\begin{definition}[Adapted from~\cite{aa-cbr,arbitrated-argumentative-dispute}] An arbitrated dispute tree is a tree $\mathcal{T}$ such that:
\label{def:arbitrated-dispute-tree}

\begin{enumerate}
    \item every node of $\mathcal{T}$ is of the form $[P:\alpha]$ for $P \in \{W, L\}$ and $\alpha \in Args$. The node is \textit{labelled} by argument $\alpha$ and assigned a status of $W$ or $L$;
    
    \item the root of $\mathcal{T}$ is labelled by the default argument, $\casedefault$, and is a:
    \begin{itemize}
        \item $W$-node if $y_{N} = \delta$,
        \item $L$-node if $y_{N} = \bar\delta$;
    \end{itemize}
    
    \item for every $W$-node $n$ labelled by some $\beta \in Args$, and for every $\gamma \in Args$ such that $\gamma \attacks \beta$, there exists a child of $n$, which is $L$-node labelled by $\gamma$;

    \item for every $L$-node $n$ labelled by some $\beta \in Args$, there exists exactly one child of $n$ which is a $W$-node labelled by some $\gamma \in Args$ such that $\gamma \attacks \beta$;

    \item There are no other nodes in $\mathcal{T}$ except those given by 1-4.
\end{enumerate}

The \textit{defence set} of $\mathcal{T}$, denoted by $\mathcal{D}(\mathcal{T})$, is the set of all arguments labelling $W$-nodes in $\mathcal{T}$.

\end{definition}

\info{ %Note to self: 
    In dispute trees \textbf{arguments label nodes} - they are not the nodes themselves
}

\unsure{Move definition to preliminaries?}


Given the scenario where $\casedefault \in \mathbb{G}$, $W$ argues in favour of acceptance of the default case. The dispute tree represents the dialectical exchange in which $W$ defends this position.

\begin{example} An arbitrated dispute tree $\mathcal{T}_{1}$ derived from the AF in Figure \ref{fig:aa-cbr-p-example} is shown in Figure \ref{fig:dispute-tree-1}. $\mathcal{T}_{1}$ showcases the dialectical exchange justifying that $y_{N_1} = +$. In this example, the root is a $W$-node, showcasing that $W$ is arguing in favour of assigning the default outcome to $N_{1}$. This dispute tree incorporates all possible explanations for the outcome predicted.  

\end{example}


\begin{figure}
    \centering
    \resizebox{.49\textwidth}{!}{
    \begin{tikzpicture}[main/.style = {}]

        \node[main] (C0) at (0, 0)  {$[W:C_{0} = (\emptyset, \emptyset, 0, + )]$};
        \node[main] (C1) at (-3, -1) {$[L:C_{1} = (\{a, b\}, \{a\}, 3, - )]$};
        \node[main] (C2) at (3, -1)  {$[L:C_{2} = (\{b, c\}, \{a\}, 1, - )]$};
        % \node[main] (C3) at (-3, -2) {$[W:C_{3} = (\{a, b\}, \{a, b\}, 2, + )]$};
        \node[main] (C4) at (-3, -2) {$[W:C_{4} = (\{a, b, c\}, \{a, c\}, 3, + )]$};
        % \node[main] (C5) at (-3, -3) {$[L:C_{5} = (\{a, b\}, \{a, b\}, 6, - )]$};
        \node[main] (C6) at (3, -3)  {$[L:C_{6} = (\{a, b, c\}, \{a, b\}, 5, - )]$};
        \node[main] (C7) at (3, -2)  {$[W:C_{7} = (\{b, c\}, \{a\}, 2, + )]$};
        % \node[main] (N1) at (-3, -4)  {$[W:N =     (\{a, b, c\}, \{a, c\}, 4, ?)]$};
        \node[main] (N1) at (3, -4)  {$[W:N_1 =     (\{a, b, c\}, \{a, c\}, 4, +)]$};
        

        

        \draw[-] (C1) -- (C0);                   
        \draw[-] (C2) -- (C0);                   
        % \draw[-] (C3) -- (C1);                   
        \draw[-] (C4) -- (C1);                   
        % \draw[-] (C4) -- (C5);                   
        % \draw[-] (C5) -- (C3);                   
        % \draw[-] (C6) -- (C3);                   
        \draw[-] (C6) -- (C7);                   
        \draw[-] (C7) -- (C2);                   
        % \draw[-] (N) -- (C3);
        % \draw[-] (N1) -- (C5);
        \draw[-] (N1) -- (C6);

    \end{tikzpicture} 
    }
    \caption{Caption $\mathcal{T}_{1}$}
    \label{fig:dispute-tree-1}
\end{figure}


In the circumstance where $\casedefault \not \in \mathbb{G}$, the arbitrated dispute tree showcases a dispute where $L$ attempts to argue in favour of acceptance of the default case but it thwarted by $W$. 

\begin{example} In contrast, a dispute tree explaining the outcome for $N_{2}$, derived from \ref{fig:aa-cbr-p-example-2}, is given in Figure \ref{fig:dispute-tree-2}. This dispute tree, $\mathcal{T}_{2}$, explains that $y_{N_2} = -$ by highlighting arguments against the $L$'s claim for the root node. This is not the only possible dispute tree. Figure \ref{fig:dispute-tree-3} shows $\mathcal{T}_{2}'$, with an alternative justification for the predicted outcome. 

\end{example}

\begin{figure}[b]
    \centering
    \resizebox{.49\textwidth}{!}{
    \begin{tikzpicture}[main/.style = {}]

        \node[main] (C0) at (0, 0)  {$[L:C_{0} = (\emptyset, \emptyset, 0, + )]$};
        \node[main] (C1) at (-3, -1) {$[W:C_{1} = (\{a, b\}, \{a\}, 3, - )]$};
        \node[main] (C2) at (3, -1)  {$[W:C_{2} = (\{b, c\}, \{a\}, 1, - )]$};
        % \node[main] (C3) at (-3, -8) {$[L:C_{3} = (\{a, b\}, \{a, b\}, 2, + )]$};
        \node[main] (C4) at (-3, -2) {$[L:C_{4} = (\{a, b, c\}, \{a, c\}, 3, + )]$};
        % \node[main] (C5) at (-3, -7) {$[W:C_{5} = (\{a, b\}, \{a, b\}, 6, - )]$};
        \node[main] (C6) at (3, -3)  {$[W:C_{6} = (\{a, b, c\}, \{a, b\}, 5, - )]$};
        \node[main] (C7) at (3, -2)  {$[L:C_{7} = (\{b, c\}, \{a\}, 2, + )]$};
        \node[main] (N2) at (-3, -3)  {$[W:N_2 =     (\{a, b, c\}, \{a, c\}, 4, -)]$};
        

        

        \draw[-] (C1) -- (C0);                   
        \draw[-] (C2) -- (C0);                   
        % \draw[-] (C3) -- (C1);                   
        \draw[-] (C4) -- (C1);                   
        % \draw[-] (C4) -- (C5);                   
        % \draw[-] (C5) -- (C3);                   
        % \draw[-] (C6) -- (C3);                   
        \draw[-] (C6) -- (C7);                   
        \draw[-] (C7) -- (C2);                   
        % \draw[-] (N) -- (C3);
        % \draw[-] (N1) -- (C5);
        \draw[-] (N2) -- (C4);

    \end{tikzpicture} 
    }
    \caption{Caption $\mathcal{T}_{2}$}
    \label{fig:dispute-tree-2}
\end{figure}


\begin{figure}[b]
    \centering
    \resizebox{.49\textwidth}{!}{
    \begin{tikzpicture}[main/.style = {}]

        \node[main] (C0) at (0, 0)  {$[L:C_{0} = (\emptyset, \emptyset, 0, + )]$};
        \node[main] (C1) at (-3, -1) {$[W:C_{1} = (\{a, b\}, \{a\}, 3, - )]$};
        \node[main] (C2) at (3, -1)  {$[W:C_{2} = (\{b, c\}, \{a\}, 1, - )]$};
        \node[main] (C3) at (-3, -2) {$[L:C_{3} = (\{a, b\}, \{a, b\}, 2, + )]$};
        \node[main] (C4) at (-3, -4) {$[L:C_{4} = (\{a, b, c\}, \{a, c\}, 3, + )]$};
        \node[main] (C5) at (-3, -3) {$[W:C_{5} = (\{a, b\}, \{a, b\}, 6, - )]$};
        \node[main] (C6) at (3, -3)  {$[W:C_{6} = (\{a, b, c\}, \{a, b\}, 5, - )]$};
        \node[main] (C7) at (3, -2)  {$[L:C_{7} = (\{b, c\}, \{a\}, 2, + )]$};
        \node[main] (N2) at (-3, -5)  {$[W:N_2 =     (\{a, b, c\}, \{a, c\}, 4, -)]$};
        

        

        \draw[-] (C1) -- (C0);                   
        \draw[-] (C2) -- (C0);                   
        \draw[-] (C3) -- (C1);                   
        % \draw[-] (C4) -- (C1);                   
        \draw[-] (C4) -- (C5);                   
        \draw[-] (C5) -- (C3);                   
        % \draw[-] (C6) -- (C3);                   
        \draw[-] (C6) -- (C7);                   
        \draw[-] (C7) -- (C2);                   
        % \draw[-] (N) -- (C3);
        % \draw[-] (N1) -- (C5);
        \draw[-] (N2) -- (C4);

    \end{tikzpicture} 
    }
    \caption{Caption $\mathcal{T}_{2}'$}
    \label{fig:dispute-tree-3}
\end{figure}


\unsure{Do I need to prove the following? They are the same proofs as in the paper}
\cite{arbitrated-argumentative-dispute} identify and prove desirable properties of arbitrated dispute trees when the casebase is coherent, justifying their choice as an explanation of an AA-CBR model. Firstly, the leaves of $\mathcal{T}$ are always $W$-nodes, and so intuitively, $W$ always `wins' the dispute. Secondly, $N$ only labels $W$-node(s) when included in $\mathcal{T}$. $N$ can, therefore, be viewed as an arbiter always agreeing with the debate's winner. Thirdly, the defence set, $\mathcal{D}(\mathcal{T})$, will always be a subset of the grounded extension $\mathbb{G}$. Thus, the winner's arguments will always be accepted and well-founded. Finally, there always exists an arbitrated dispute tree with $W$ assigned to the root if $\casedefault \in \mathbb{G}$ and $L$ assigned to the root if \mbox{$\casedefault \not \in \mathbb{G}$ 
\footnote{Note that this last property is stronger than that identified by~\cite{arbitrated-argumentative-dispute}, in which the dispute trees for AA-CBR with Stages were used to explain known outcomes, not predicted outcomes. As a result, in situations where $\casedefault \in \mathbb{G}$ and $y_{n} \neq \delta$ (or $\casedefault \not \in \mathbb{G}$ and $y_{n} = \delta$), an arbitrated dispute tree could not be derived. AA-CBR-$P_{\succcurlyeq}$ does not suffer this issue as the outcome assigned to $N$ is always determined by the status of $\casedefault$ in $\mathbb{G}$.}.}


When the casebase is incoherent, an arbitrated dispute tree is not guaranteed to exist. 
\begin{example}
Consider the AF in Figure \ref{fig:incoherent-dispute}. The grounded extension for this framework is $\mathbb{G} = \{N\}$. If we attempt to construct a dispute tree from the AF, a node labelled with $C_0$ would be the root and assigned status $L$. Due to condition 4. of Definition \ref{def:arbitrated-dispute-tree}, this root node must have a $W$-node child, but $C_{1}$ cannot label a $W$-node as we know that $\mathcal{D}(\mathcal{T}) \subseteq \mathbb{G}$ and $C_{1} \not \in \mathbb{G}$. 

\end{example}

\begin{figure}
    \centering
    \resizebox{.49\textwidth}{!}{
    \begin{tikzpicture}[main/.style = {draw, rectangle}]

        \node[main, label=left:$C_0$] (C0) at (0, 0)  {$(\emptyset, \emptyset, 0, + )$};
        \node[main, label=left:$C_1$] (C1) at (-2, 2) {$(\{a, b\}, \{a\}, 3, - )$};
        \node[main, label=left:$C_2$] (C2) at (2, 2)  {$(\{a, b\}, \{a\}, 3, + )$};
        \node[main, label=left:$N$] (N) at (-2, 4)  {$(\{a, b, c\}, \{a, c\}, 4, ?)$};
        
        \node[] (l1) at (-7, 0)  {}; 
        \node[] (l2) at (-5, 0) {Attacks}; 
        \draw[-{Latex[length=2mm, width=3mm]}]  (l2) -- (l1);
        
        \node[] (l3) at (-7, 1)  {}; 
        \node[] (l4) at (-5, 1) {Irrelevance}; 

        

        \draw[-{Latex[length=2mm, width=3mm]}] (C1) -- (C0);                   
        \draw[-{Latex[length=2mm, width=3mm]}] (C2) to[out=135,in=45,distance=1cm] (C1);                   
        \draw[-{Latex[length=2mm, width=3mm]}] (C1) to[out=-45,in=-135,distance=1cm] (C2);
        
        \begin{scope}[transparency group, opacity=0.5]
            \draw[-{Latex[length=2mm, width=3mm]}, red, dashed] (l4) -- (l3);
        \end{scope}

    \end{tikzpicture} 
    }
    \caption{Caption}
    \label{fig:incoherent-dispute}
\end{figure}

\todoin{
\begin{itemize}
    \item Excess Features 
    \begin{itemize}
        \item We would need to modify excess features to identify the change between two cases that lead to an attack. 
        \item Originally proposed, excess features is only defined for the focus case and a parent in the dispute tree, do we want that? Or would it be good to define it for all attacks? 
    \end{itemize}
\end{itemize}
}




